Assessing Y-Axis Influence: Bias in Multimodal Language Models on Chart-to-Table Translation

Chart-to-table translation converts chart images into structured tabular data. Accurate translation is crucial for Multimodal Language Model (MLM) to answer complex queries. We observe imbalances in the number of images across different aspects of the y-axis information in public chart datasets. Such imbalances can introduce unintended biases, causing uneven MLM performance. Previous works have not systematically examined these biases. To address this gap, we propose a new framework, FairChart2Table, for analyzing y-axis-related bias on five state-of-the-art models. Key Findings: (1) There are significant y-axis biases related to the digit length of the major tick values, the number of major ticks, the range of values, and the tick value format (e.g., abbreviation or scientific format). (2) The number of legends/entities in chart images impacts MLM performance. (3) Prompting MLM with y-axis information can significantly enhance the performance for some MLMs.

==> latex/unused_sentences.tex <==
\iffalse
We conduct experiments using three different LLMs on two different datasets, and the three different types of questions are applied for every question. For each question, we calculate two metrics: final selection accuracy and reasoning accuracy. Greedy decoding is utilized for generating responses, but due to the variability of LLMs accuracy fluctuates across trials. To address this, we apply the Wilcoxon signed-rank test to assess if the differences in accuracy across question types are statistically significant. The distributions of annotated outputs, which contain 0 (incorrect) and 1 (correct) are compared.
\fi
